Self-training Room Layout Estimation via Geometry-aware Ray-casting

In this paper, we introduce a novel geometry-aware self-training framework for room layout estimation models on unseen scenes with unlabeled data. Our approach utilizes a ray-casting formulation to aggregate multiple estimates from different viewing positions, enabling the computation of reliable pseudo-labels for self-training. In particular, our ray-casting approach enforces multi-view consistency along all ray directions and prioritizes spatial proximity to the camera view for geometry reasoning. As a result, our geometry-aware pseudo-labels effectively handle complex room geometries and occluded walls without relying on assumptions such as Manhattan World or planar room walls. Evaluation on publicly available datasets, including synthetic and real-world scenarios, demonstrates significant improvements in current state-of-the-art layout models without using any human annotation.

==> fig_src/banner.tex <==
\twocolumn[{
\maketitle
\begin{center}
    \vspace{-10mm}
    \captionsetup{type=figure}
   \includegraphics[ width=\linewidth]
    {fig/banner/banner_v3.1.png}

    \begin{picture}(0, 0)
    
    \put(-235,3){(a) Multi-view Layout Estimates}
    
    \put(-60,3){(b) Ours MLC++ Pseudo-label}
    
    \put(100,3){(c) 360-MLC~\cite{360_mlc} Pseudo-label}
    
    \end{picture}
    
    \caption{By leveraging multiple estimates from a pre-trained model as presented in panel (a), MLC++ leverages a ray-casting data aggregation process to estimate geometry-aware pseudo-labels for self-training, as depicted in panel (b), i.e., pseudo-labels that encompass a comprehensive representation of the room geometry directly from unlabeled data. In comparison with previous solutions as presented in (c), where multiple estimations are processed on the image domain without geometry reasoning, MLC++ excels in defining better pseudo-labels, especially for occluded geometry, highlighting the significance of our contribution.}
    \label{fig_banner}
\end{center}
}]

==> fig_src/fig_multi_ray_casting.tex <==
\begin{figure}[t!]
  \centering
%   \includegraphics[clip, trim=0.0cm 27.0cm 42.0cm 0.0cm, width=8cm]
% {fig/ray_casting/ray_casting_v3.0.pdf}
\includegraphics[width=\linewidth]
{fig/multi_ray_casting_fig/multi_ray_casting_v0.0.png}
    \begin{picture}(0, 0)
    \put(-112,0){(a)}
    \put(-2,0){(b)}
    \put(108,0){(c)}
    \end{picture}
  \caption{\textbf{Weighted-distance function:} In panel (a), we illustrate our proposed weighted-distance function $\omega_i$ that prioritizes the farthest geometries in the scene for self-training. In panel (b), under the same scale as (a), we show the $L1$ loss between our proposed pseudo-label and the model estimation. Note that the $L1$ loss evaluation presents a small range w.r.t $\omega_i$ and does not aim at any particular region in the scene. In Panel (c), we present our pseudo-label (magenta line) and the model estimation (green line).}
  \label{fig_multi_ray_cast}
  \vspace{-5mm}
\end{figure}

==> fig_src/qualitative_bev_v2.tex <==
\begin{figure*}
    \small
    \centering
    \footnotesize
    \begin{tabular}{c c c c}
    
        % ##############################    
        % \includegraphics[clip, trim=10.5cm 25cm 10.5cm 3cm,width=0.15\linewidth,angle=-90,origin=l]{fig/qualitative_bev/bev_1LXtFkjw3qL_0_room9.png}
        % \includegraphics[clip, trim=7cm 40cm 0cm 40cm,height=0.15\linewidth]{fig/qualitative_bev/bev_8WUmhLawc2A_0_room16.png}
        % \includegraphics[clip, trim=10cm 10cm 17cm 20cm,width=0.15\l  inewidth,angle=-90,origin=l]{fig/qualitative_bev/bev_ac26ZMwG7aT_0_room3.png}
        % \includegraphics[clip, trim=0cm 40cm 10cm 40cm, height=0.15\linewidth]{fig/qualitative_bev/bev_FgswoxWb3uN_1_room0.png}
        % \\

        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/bev_1LXtFkjw3qL_0_room9.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/bev_8WUmhLawc2A_0_room16.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/bev_ac26ZMwG7aT_0_room3.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/bev_FgswoxWb3uN_1_room0.png}
        \\
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/mlc_1LXtFkjw3qL_0_room9.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/mlc_8WUmhLawc2A_0_room16.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/mlc_ac26ZMwG7aT_0_room3.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/mlc_FgswoxWb3uN_1_room0.png}
        \\

        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/xyz_lys_wc_1LXtFkjw3qL_0_room9.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/xyz_lys_wc_8WUmhLawc2A_0_room16.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/xyz_lys_wc_ac26ZMwG7aT_0_room3.png}
        \includegraphics[width=0.18\linewidth]{fig/qualitative_bev/xyz_lys_wc_FgswoxWb3uN_1_room0.png}
        \\
        
    \end{tabular}
    \caption{
        \textbf{Qualitative comparisons of estimated pseudo-labels.} We show a BEV projection of all layout geometries in the scene. Column (a) shows all layout estimates from a pre-trained model \cite{horizonnet}, column (b) all pseudo-labels from 360-MLC\cite{360_mlc}, and column (c) our proposed MLC++.}
    
    \label{fig_qualitative_bev}
\end{figure*}


==> fig_src/qualitative_fig.tex <==
\begin{figure*}
    \small
    \centering
    \footnotesize
    \begin{tabular}{c c c}
    
        % ##############################    
        \includegraphics[page=9, width=0.3\linewidth]{fig/qualitative_on_equi/h1zeeAwLh9Z_2_room0_52.jpg}

        \includegraphics[page=7, width=0.3\linewidth]{fig/qualitative_on_equi/7y3sRwLe3Va_0_room0_10355.jpg}
        
        \includegraphics[page=4, width=0.3\linewidth]{fig/qualitative_on_equi/1103_floor_01_partial_room_07_pano_7.jpg}

        % ##############################    
        \\
        \includegraphics[page=10, width=0.3\linewidth]{fig/qualitative_on_equi/mL8ThkuaVTM_4_room0_42.jpg}

        \includegraphics[page=8, width=0.3\linewidth]{fig/qualitative_on_equi/7y3sRwLe3Va_0_room0_7873.jpg}

        \includegraphics[page=2, width=0.3\linewidth]{fig/qualitative_on_equi/0375_floor_01_partial_room_09_pano_15.jpg} 

        % ##############################    
        \\
        \includegraphics[page=11, width=0.3\linewidth]{fig/qualitative_on_equi/rJhMRvNn4DS_0_room0_50.jpg}

        \includegraphics[page=13, width=0.3\linewidth]{fig/qualitative_on_equi/VFuaQ6m2Qom_0_room4_13933.jpg}
        
        \includegraphics[page=3, width=0.3\linewidth]{fig/qualitative_on_equi/1103_floor_01_partial_room_07_pano_10.jpg}
        \\
        \\


    % HM3D-MVL
    % \includegraphics[page=14, width=0.3\linewidth]{fig/qualitative_on_equi/wcojb4TFT35_2_room0_146.jpg}

    % ZIND-MVL
    % \includegraphics[page=1, width=0.3\linewidth]{fig/qualitative_on_equi/0181_floor_01_partial_room_01_pano_30.jpg}
    
    %  \includegraphics[page=5, width=0.3\linewidth]{fig/qualitative_on_equi/1330_floor_01_partial_room_09_pano_22.jpg}
    
    % \includegraphics[page=6, width=0.3\linewidth]{fig/qualitative_on_equi/6D36GQHuP8H_1_room0_22.jpg}
    \end{tabular}
    
    \begin{picture}(0, 0)
    
    \put(-180,3){(a) Our HM3D-MVL}
    
    \put(-30,3){(b) MP3D-FPE \cite{360_dfpe}}
    
    \put(140,3){(c) ZInD \cite{zind}}
    
    \end{picture}
    \caption{
        \textbf{Qualitative comparisons on panoramic images.}. The results in this figure present: a pre-trained model \cite{horizonnet} (orange line), self-training 360-MLC~\cite{360_mlc} (cyan line), and our proposed MLC++ (magenta line). 
        % In column (a) our proposed dataset \textbf{HM3D-MVL}, column (b) MP3D-FPE \cite{360_dfpe}, and column (c) ZInD \cite{zind}.  
    }
    \label{fig_qualitative_pano}
\end{figure*}


==> fig_src/ray_casting_alg.tex <==
\begin{algorithm}
\caption{MLC++: Ray-Casting Pseudo Labeling}\label{alg:ray_cast_alg}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\Require
~~Layout estimates 
$\mathbf{Y}\in\mathbb{R}^{3\times nW}$ defined by \cref{eq_ly_concat}

Set of ray vectors $\mathcal{R}$ and $\mathcal{V}$ defined by \cref{eq_ray_directions}

% Set cam poses~$\mathcal{T}=\{[\mathbf{R}_i|\mathbf{t_i}]\in SE(3)\}_{i=0:n}$
\Ensure 
Pseudo-labels per view in the scene $\{\mathbf{\bar{y}}_i\}_{i=1:n}$
\For {each cycle $k$}\Comment{Filtering Noisy Estimates}

\State $\mathcal{Q}\gets \varnothing$

\For {each view $i$}\Comment{Loop per view in the scene}

\State $\mathbf{Y}_i \gets \mathbf{R}_i~\mathbf{Y} + \mathbf{t}_i$

\For {each $\mathbf{r}\in$}\Comment{Loop per ray direction}

\State $\mathcal{Q}\gets \mathcal{Q} \cup \{median(\Omega_r(\mathbf{Y}_i)\mathbf{r}\}$
\EndFor
\EndFor
\State $\mathbf{Y}\gets \mathbf{q}_1 \cup \cdots \cup \mathbf{q}_w$,~~~$\mathbf{q}\in\mathcal{Q}$,~~$\mathbf{q}\in\mathbb{R}^3$ 
\EndFor

\State $\mathcal{Q}\gets \varnothing$
\For {each view $i$}\Comment{Estimating Pseudo-labels}
\State $\mathbf{Y}_i \gets \mathbf{R}_i~\mathbf{Y} + \mathbf{t}_i$

\For {each $\mathbf{r}\in \mathcal{R}$}
\State $\mathcal{Q}\gets \mathcal{Q} \cup \{min(\mathbf{r}\cdot\mathbf{Y}_i) ~~\mathbf{r}\}$
\EndFor
\State $\mathbf{\bar{y}}_i\gets \mathbf{q}_1 \cup \cdots \cup \mathbf{q}_w$,~~~$\mathbf{q}\in\mathcal{Q}$,~~$\mathbf{q}\in\mathbb{R}^3$ 
\EndFor
\end{algorithmic}
\end{algorithm}
\vspace{-2mm}

==> section/3_method/algorithm.tex <==
\begin{algorithm}
\caption{MLC++: Ray-Casting Pseudo Labeling}\label{alg:ray_cast_alg}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\Require
~~Layout estimates 
$\mathbf{Y}\in\mathbb{R}^{3\times nW}$ defined by \cref{eq_ly_concat}

Set of ray vectors $\mathcal{R}$ and $\mathcal{V}$ defined by \cref{eq_ray_directions}

% Set cam poses~$\mathcal{T}=\{[\mathbf{R}_i|\mathbf{t_i}]\in SE(3)\}_{i=0:n}$
\Ensure 
Pseudo-labels per view in the scene $\{\mathbf{\bar{y}}_i\}_{i=1:n}$
\For {each cycle $k$}\Comment{Filtering Noisy Estimates}

\State $\mathcal{Q}\gets \varnothing$

\For {each view $i$}\Comment{Loop per view in the scene}

\State $\mathbf{Y}_i \gets \mathbf{R}_i~\mathbf{Y} + \mathbf{t}_i$

\For {each $\mathbf{r}\in$}\Comment{Loop per ray direction}

\State $\mathcal{Q}\gets \mathcal{Q} \cup \{median(\Omega_r(\mathbf{Y}_i)\mathbf{r})\}$
\EndFor
\EndFor
\State $\mathbf{Y}\gets \mathbf{q}_1 \cup \cdots \cup \mathbf{q}_w$,~~~$\mathbf{q}\in\mathcal{Q}$,~~$\mathbf{q}\in\mathbb{R}^3$ 
\EndFor

\State $\mathcal{Q}\gets \varnothing$
\For {each view $i$}\Comment{Estimating Pseudo-labels}
\State $\mathbf{Y}_i \gets \mathbf{R}_i~\mathbf{Y} + \mathbf{t}_i$

\For {each $\mathbf{r}\in \mathcal{R}$}
\State $\mathcal{Q}\gets \mathcal{Q} \cup \{min(\mathbf{r}\cdot\mathbf{Y}_i) ~~\mathbf{r}\}$
\EndFor
\State $\mathbf{\bar{y}}_i\gets \mathbf{q}_1 \cup \cdots \cup \mathbf{q}_w$,~~~$\mathbf{q}\in\mathcal{Q}$,~~$\mathbf{q}\in\mathbb{R}^3$ 
\EndFor
\end{algorithmic}
\end{algorithm}
\vspace{-2mm}

==> table/exp_ab_data.tex <==
\begin{table*}
\fontsize{8.8}{12}\selectfont
  \caption{Ablation study on the amount of training data.}
  \label{exp_ab_data}
  \centering
  \begin{tabular}{ll cc cc cc cc}
    \toprule
    
    & & \multicolumn{4}{c}{10\%} & \multicolumn{2}{c}{60\%} & \multicolumn{2}{c}{100\%}\\
    Dataset & Method & 2D IoU (\%) $\uparrow$ & 3D IoU (\%) $\uparrow$ & 2D IoU (\%) $\uparrow$ & 3D IoU (\%) $\uparrow$ & 2D IoU (\%) $\uparrow$ & 3D IoU (\%) $\uparrow$ \\
    
    \midrule
    
    \multirow{2}{*}{HM3D-MVL~\cite{hm3d}}
        & 360-MLC~\cite{360_mlc} \\
        & Ours \\

    \midrule

    \multirow{2}{*}{MP3D-FPE~\cite{360_dfpe}}
        & 360-MLC \\
        & Ours \\

    \midrule

    \multirow{2}{*}{ZInD~\cite{zind}}
        & 360-MLC \\
        & Ours \\
    
    \bottomrule
  \end{tabular}
\end{table*}

==> table/exp_ab_data_v2.tex <==
\begin{table*}
\fontsize{8.8}{12}\selectfont
  \caption{Ablation study on the amount of training data.}
  \label{exp_ab_data}
  \centering
  \begin{tabular}{ll cc | cc}
    \toprule

    & & \multicolumn{2}{c}{2D IoU (\%) $\uparrow$} & \multicolumn{2}{c}{3D IoU (\%) $\uparrow$} \\
    
    Dataset & Method &
    10\% & 100\% &
    10\% & 100\% \\

    \midrule
    
    \multirow{2}{*}{HM3D-MVL~\cite{hm3d}}
        & 360-MLC~\cite{360_mlc}
        &81.66	&79.19	&80.08	&77.72\\
        & Ours 
        &82.05	&83.01	&80.45	&81.38
        \\

    \midrule

    \multirow{2}{*}{MP3D-FPE~\cite{360_dfpe}}
        & 360-MLC
        &84.15	&83.95	&82.27	&82.04\\
        & Ours
        &85.21	&85.71	&83.16	&83.58\\

    \midrule

    \multirow{2}{*}{ZInD~\cite{zind}}
        & 360-MLC
        &62.04	&63.33	&59.29	&60.47\\
        & Ours
        &62.72	&64.01	&60.12	&61.37\\
    
    \bottomrule
  \end{tabular}
\end{table*}

==> table/exp_ab_dwL1_10and100.tex <==
\begin{table}[!t]
\vspace{5mm}
\fontsize{8.5}{10}\selectfont
  \caption{Ablation study for our weighted-distance loss using HM3D-MVL dataset.
  % losses. PT stands for Pre-Trained. WD stands for Weighting Distance (Our full MLC++).
  }
  \vspace{-2mm}
  \label{tab_ablation}
  \centering
  \begin{tabular}{ll c c | c c | c c | c c}
    \toprule
     && \multicolumn{2}{c|}{Testing set} & \multicolumn{2}{c}{Occlusion Subset} &
     \multicolumn{2}{c|}{Testing set} & \multicolumn{2}{c}{Occlusion Subset} \\
     & Loss  & 2D IoU~$\uparrow$ & 3D IoU~$\uparrow$ & 2D Io~$\uparrow$ & 3D IoU~$\uparrow$ \\
    \midrule
    (a)& Pre-trained~\cite{horizonnet} &76.71	&71.79	&78.74&	75.72\\ 
    (b)& Pseudo-labels &81.65& 76.99 &80.85	&78.98\\
    (c)& $\omega$=$\sigma^{-2}$ &
    81.02	&76.58	&81.28	&79.53\\
    % (d)& $\omega=sin(\sigma^{-2}_{bev})$.& 
    % 81.01	&77.31	&81.97	&80.19\\
    (d)& $\omega$ = \cref{eq_w_fucntion}  
    &\textbf{81.74}	&\textbf{77.99}	
    &\textbf{82.05}	&\textbf{80.45}\\ 
    \bottomrule
  \end{tabular}
  \vspace{-5mm}
\end{table}
%\cref{eq_w_fucntion}
% \vspace{-3mm}


==> table/exp_ab_policy.tex <==
\begin{table*}
\fontsize{9}{12}\selectfont
  \caption{Ablation study on policy.}
  \label{exp_ab_policy}
  \centering
  \begin{tabular}{ll c c c c}
    \toprule
    
    Dataset & Policy & 2D IoU (\%) $\uparrow$ & 3D IoU (\%) $\uparrow$ & RMSE $\downarrow$ & $\delta_1 \uparrow$ \\
    
    \midrule
    
    \multirow{2}{*}{HM3D-MVL~\cite{hm3d}}
        & random \\
        & stable \\
        & large difference \\
        & stable + large difference \\

    \midrule

    \multirow{2}{*}{MP3D-FPE~\cite{360_dfpe}}
        & random \\
        & stable \\
        & large difference \\
        & stable + large difference \\

    \midrule

    \multirow{2}{*}{ZInD~\cite{zind}}
        & random \\
        & stable \\
        & large difference \\
        & stable + large difference \\
    
    \bottomrule
  \end{tabular}
\end{table*}

==> table/exp_ab_policy_all_vs_occlusion.tex <==
\begin{table*}
\fontsize{9}{12}\selectfont
  \caption{Ablation study on policy.}
  \label{exp_ab_policy}
  \centering
  \begin{tabular}{l l c c c c}
    \toprule
    & \multicolumn{2}{c}{Testing set} & \multicolumn{2}{c}{Occlusion subset}\\
    & Policy & 2D IoU (\%) $\uparrow$ & 3D IoU (\%) $\uparrow$ & 2D IoU (\%) $\uparrow$ & 3D IoU (\%) $\uparrow$  \\
    \midrule
    
    (a) & random \\
    (b) & stable \\
    (c) & large difference \\
    (d) & (b) + (c) \\    
    
    \bottomrule
  \end{tabular}
\end{table*}

==> table/exp_main.tex <==
\begin{table*}
\fontsize{9}{12}\selectfont
  \caption{Main experiment.}
  \label{exp_main}
  \centering
  \begin{tabular}{ll c c | c c}
    \toprule
    && \multicolumn{2}{c|}{Testing set} & \multicolumn{2}{c}{Occlusion Subset}\\
    Dataset & Method & 2D IoU (\%) $\uparrow$ & 3D IoU (\%) $\uparrow$ & 2D IoU (\%) $\uparrow$ & 3D IoU (\%)
    $\uparrow$\\
    
    \midrule
    
    \multirow{3}{*}{HM3D-MVL~\cite{hm3d}}
        & Pre-trained \cite{horizonnet} & 78.90	& 74.04&  40.91	8.63876.71 & 71.79 & 78.74 & 75.72\\
        & 360-MLC~\cite{360_mlc} &82.71 &78.71 
        &79.19 &77.72\\
        & MLC++ & sdsd
        82.99	&78.95	&83.01	&81.38\\
        
    \midrule

    \multirow{3}{*}{MP3D-FPE~\cite{360_dfpe}}
        & Pre-trained & 77.33 & 74.07 & 
        75.09 & 73.36 \\
        & 360-MLC & 80.93 &	77.69 &
        84.27 & 82.04\\
        & MLC++ & 81.65 &	78.21 &
        85.71 & 83.58\\
        
    \midrule

    \multirow{3}{*}{ZInD~\cite{zind}}
        & Pre-trained & 69.63 & 65.54 & 59.98 &	53.95\\
        & 360-MLC & 75.44	& 72.28 &
        63.33 & 60.47\\
        & MLC++ & 76.71 &	73.04 &
         64.01 & 61.37\\ 
        
    \bottomrule
  \end{tabular}
\end{table*}
